Higher criticism for rare and weak non-proportional hazard deviations in survival analysis

We propose a method for comparing survival data based on the higher criticism of p-values obtained from multiple exact hypergeometric tests. The method accommodates non-informative right-censorship and is sensitive to hazard differences in unknown and relatively rare time intervals. It attains much better power against such differences than the log-rank test and its variants. We demonstrate the usefulness of our method in detecting rare and weak non-proportional hazard differences compared to existing tests, using simulations and actual gene expression data. Additionally, we analyze the asymptotic power of our method and other tests under a theoretical framework describing two groups experiencing failure rates that are usually identical over time, except in a few unknown instances where one group's failure rate is higher. Our test's power undergoes a phase transition across the plane of rarity and intensity parameters that mirrors the phase transition of higher criticism in two-sample settings with rare and weak normal and Poisson means. The region of the plane in which our method has asymptotically full power is larger than the corresponding region for the log-rank test.

==> table_critical_values.tex <==
\begin{table}[ht]
    \begin{center}
    \begin{tabular}{|c|c||c|c|}
    \toprule
          & $T$ & $q_0^{0.95}(\HCHG)$ & $q_0^{0.95}(\LR)$ \\
        \midrule
        %\rule{0pt}{9pt}
         %  exponential decay
         %   & 
         %  $100$ & $1500$ & $0.14$ & $0.48$ $(0.02)$ & $1.94$ $(0.02)$ \\ 
         % ($H_0$ of \eqref{eq:sampling_model}) 
         % %& $100$ & $1500$ & $2$ & $2.88$ $(0.06)$ & $2.04$ $(0.02)$ \\ 
         %  & 
         %  $1000$ & $10000$ & $5$ & $1.77$ $( 0.05)$ & $1.96$ $(0.02)$ \\ 
         % % & $2000$ & $20000$ & $5$ & $1.77$ $(0.06)$ & $1.97$ $(0.02)$ \\
         %  \hline 
          random group assignment
          & $82$ & $0.29$ $ (0.07)$ 
          & $1.55$ $(0.02)$ 
\\
           & $100$ &
         $-0.06$ $(0.01)$ &
         $1.57$ $(0.01)$ \\
          %& $200$ & $1534$ $(28.1)$ & $6.1$ $(0.37)$ &  -1.17 (0.014) & $1.77$ $(0.018)$ \\
          %& $500$ & $1534$ $(27.7)$ & $6.5$ $(0.40)$ &  $-5.06$ $(0.02)$ & $1.79$ $(0.02)$
          
           & $200$ &
         $-1.21$ $(0.01)$ &
         $1.56$ $(0.02)$ \\
        \hline 
         uniform P-values & $100$ & $1.88$ $(0.01)$ & \\
         ($p_t \sim \mathrm{Unif}(0,1)$) 
          & $1000$ & $2.36$ $(0.02)$ & \\
          %& $10000$ & $2.64$ %$(0.02)$ & \\
          \hline
          % asymptotic distribution & $100$ & $3.24$ & $1.68$ \\ 
          %%& $500$ & & & $3.32$ & %$1.68$ \\ 
          %& $1000$ & $3.35$ & %$1.68$ \\ 
          %& $10000$ & $3.43$ & %$1.68$ \\ 
    \end{tabular}
    \end{center}
    \caption{
    Critical values for testing at significance level $\alpha=0.05$. Top block: $1-\alpha$ quantile of a sample obtained by 
    randomly assigning groups in the gene expression data. Bottom: Simulated $1-\alpha$ quantile of values of HC of uniform P-values. 
    We report on the standard errors of quantile estimates in brackets as obtained using a Maritz-Jarrett type estimator\cite{maritz1978note} and verified via bootstrapping.
    }
    \label{tlbl:critical_values}
\end{table}

==> table_large_pvals.tex <==

% Setup siunitx:
\sisetup{
  round-mode          = places, % Rounds numbers
  round-precision     = 2, % to 2 places
}

\pgfplotstableset{ % Makes bold a whole row of a table
    highlightrow/.style={
        postproc cell content/.append code={
           \count0=\pgfplotstablerow
            \advance\count0 by1
            \ifnum\count0=#1
            \pgfkeysalso{@cell content/.add={$\bf}{$}}
            \fi
        },
    },
}

\begin{table}
    \begin{tikzpicture} 
    
    \node[left, scale=.8] (table) at (-1.2,-7.4) {      
    \pgfplotstabletypeset[
      multicolumn names, 
      col sep=comma, 
      display columns/0/.style={
        column name= $t-1$, 
        column type={l},string type}, 
      display columns/1/.style={
        column name=$n_x(t-1)$,
        column type={l},string type},
      display columns/2/.style={
        column name=$n_y(t-1)$,
        column type={l},string type},        
    display columns/3/.style={
         column name= $o_x(t)$,
         column type={l},string type},
    display columns/4/.style={
        column name= $o_y(t)$,
        column type={l},string type},
    display columns/5/.style={
        column name= $p_{t}$,
        column type={l},string type},
    every head row/.style={
        before row={\toprule}, % have a rule at top
        after row={
            %$t$ & $N_x$ & N_y & O_x & O_y & $p$ \\ % the units seperated by &
            \midrule} % rule under units
            },
    highlightrow/.style={
        postproc cell content/.append code={
            \count0=\pgfplotstablerow
            \advance\count0 by1
            \ifnum\count0=#1
                \pgfkeysalso{@cell content=\textbf{##1}}
            \fi
            },
        },
    every last row/.style={after row=\bottomrule}, % rule at bottom
        ] {csv/survival_curve_exm_low_rate.csv}};
\end{tikzpicture}

\begin{center}
    \caption{
    Hypergeometric P-values for data sampled from \eqref{eq:model_full} when the risk rate $\bar{\lambda}$ is small.  }
    \end{center}
    \label{tbl:large_pvals}
\end{table}

